Multi-Bracket High Dynamic Range Imaging with Event Cameras

Modern high dynamic range (HDR) imaging pipelines align and fuse multiple low dynamic range (LDR) images captured at different exposure times. While these methods work well in static scenes, dynamic scenes remain a challenge since the LDR images still suffer from saturation and noise. In such scenarios, event cameras would be a valid complement, thanks to their higher temporal resolution and dynamic range. In this paper, we propose the first multi-bracket HDR pipeline combining a standard camera with an event camera. Our results show better overall robustness when using events, with improvements in PSNR by up to 5dB on synthetic data and up to 0.7dB on real-world data. We also introduce a new dataset containing bracketed LDR images with aligned events and HDR ground truth.

==> floats/fig_eye_catcher.tex <==
\global\long\def\figHeight{3.54cm}
\makeatletter
\let\@oldmaketitle\@maketitle% Store \@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle% Update \@maketitle to insert...
    \vspace{-6mm}
    \includegraphics[height=\figHeight]{floats/images/flag.png}
    \vspace{-7mm}
    \captionof{figure}{We propose to leverage the high dynamic range properties of an event camera to enhance a multi-bracket pipeline for HDR imaging. 
    Events substantially improve the alignment of LDR images in scenes with both object and camera motion.
    \vspace{4mm}} \label{fig:eye}
}% ... an image
\makeatother
% \vspace{20mm}

==> floats/fig_flag.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=0.97\textwidth]{floats/images/flag.png}
\caption{Qualitative comparison of our method against state-of-the-art works on the real dataset. Crops emphasize details.}\label{fig:qual_flag}
\end{figure*} 

